You Don't Need All Attentions: Distributed Dynamic Fine-Tuning for Foundation Models

Fine-tuning plays a crucial role in adapting models to downstream tasks with minimal training efforts. However, the rapidly increasing size of foundation models poses a daunting challenge for accommodating foundation model fine-tuning in most commercial devices, which often have limited memory bandwidth. Techniques like model sharding and tensor parallelism address this issue by distributing computation across multiple devices to meet memory requirements. Nevertheless, these methods do not fully leverage their foundation nature in facilitating the fine-tuning process, resulting in high computational costs and imbalanced workloads. We introduce a novel Distributed Dynamic Fine-Tuning (D2FT) framework that strategically orchestrates operations across attention modules based on our observation that not all attention modules are necessary for forward and backward propagation in fine-tuning foundation models. Through three innovative selection strategies, D2FT significantly reduces the computational workload required for fine-tuning foundation models. Furthermore, D2FT addresses workload imbalances in distributed computing environments by optimizing these selection strategies via multiple knapsack optimization. Our experimental results demonstrate that the proposed D2FT framework reduces the training computational costs by 40% and training communication costs by 50% with only 1% to 2% accuracy drops on the CIFAR-10, CIFAR-100, and Stanford Cars datasets. Moreover, the results show that D2FT can be effectively extended to recent LoRA, a state-of-the-art parameter-efficient fine-tuning technique. By reducing 40% computational cost or 50% communication cost, D2FT LoRA top-1 accuracy only drops 4% to 6% on Stanford Cars dataset.

==> math.tex <==
\usepackage{bbm}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{hypothesis}{Hypothesis}

\newtheorem{property}{Property}
\newtheorem{conjecture}{Conjecture}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{condition}{Condition}
\newtheorem{fact}{Fact}
% \newtheorem{procedure}{Procedure}
\newtheorem{assumption}{Assumption}
% \newenvironment{proof}{\paragraph*{Proof}}{\hfill$\square$}

\newenvironment{densitemize}%    Densely printed itemized list,
{\begin{list}               %    with flush left bullets.
    {$\bullet$ \hfill}{
        \setlength{\leftmargin}{\parindent}
        \setlength{\parsep}{0.04\baselineskip}
        \setlength{\itemsep}{0.5\parsep}
        \setlength{\labelwidth}{\leftmargin}
        \setlength{\labelsep}{0em}}
    }
{\end{list}}

\providecommand{\eref}[1]{\eqref{#1}}  % call \eqref from amstex
\providecommand{\cref}[1]{Chapter~\ref{#1}}
\providecommand{\sref}[1]{Section~\ref{#1}}
\providecommand{\fref}[1]{Figure~\ref{#1}}
\providecommand{\tref}[1]{Table~\ref{#1}}
\providecommand{\thref}[1]{Theorem~\ref{#1}}

\providecommand{\R}{\ensuremath{\mathbb{R}}}
\providecommand{\I}{\ensuremath{\mathbb{I}}}
\providecommand{\C}{\ensuremath{\mathbb{C}}}
\providecommand{\E}{\ensuremath{\mathbb{E}}}
\providecommand{\N}{\ensuremath{\mathbb{N}}}
\providecommand{\Z}{\ensuremath{\mathbb{Z}}}
\providecommand{\Pb}{\ensuremath{\mathbb{P}}}

\providecommand{\bfP}{\mathbf{P}}

\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\inprod}[1]{\langle#1\rangle}
\providecommand{\set}[1]{$\left\{#1\right\}$}
\providecommand{\seq}[1]{$\left<#1\right>$}
\providecommand{\bydef}{\overset{\text{def}}{=}}

\renewcommand{\vec}[1]{\ensuremath{\boldsymbol{#1}}}
\providecommand{\mat}[1]{\ensuremath{\boldsymbol{#1}}}


% Some calligraphic letters
\providecommand{\calA}{\mathcal{A}}
\providecommand{\calB}{\mathcal{B}}
\providecommand{\calC}{\mathcal{C}}
\providecommand{\calD}{\mathcal{D}}
\providecommand{\calE}{\mathcal{E}}
\providecommand{\calF}{\mathcal{F}}
\providecommand{\calG}{\mathcal{G}}
\providecommand{\calH}{\mathcal{H}}
\providecommand{\calI}{\mathcal{I}}
\providecommand{\calJ}{\mathcal{J}}
\providecommand{\calK}{\mathcal{K}}
\providecommand{\calL}{\mathcal{L}}
\providecommand{\calM}{\mathcal{M}}
\providecommand{\calN}{\mathcal{N}}
\providecommand{\calO}{\mathcal{O}}
\providecommand{\calP}{\mathcal{P}}
\providecommand{\calQ}{\mathcal{Q}}
\providecommand{\calR}{\mathcal{R}}
\providecommand{\calS}{\mathcal{S}}
\providecommand{\calT}{\mathcal{T}}
\providecommand{\calU}{\mathcal{U}}
\providecommand{\calV}{\mathcal{V}}
\providecommand{\calW}{\mathcal{W}}
\providecommand{\calX}{\mathcal{X}}
\providecommand{\calY}{\mathcal{Y}}
\providecommand{\calZ}{\mathcal{Z}}


% Common matrices and vectors
\providecommand{\mA}{\mathbf{A}}
\providecommand{\mB}{\mathbf{B}}
\providecommand{\mC}{\mathbf{C}}
\providecommand{\mD}{\mathbf{D}}
\providecommand{\mE}{\mathbf{E}}
\providecommand{\mF}{\mathbf{F}}
\providecommand{\mG}{\mathbf{G}}
\providecommand{\mH}{\mathbf{H}}
\providecommand{\mI}{\mathbf{I}}
\providecommand{\mJ}{\mathbf{J}}
\providecommand{\mK}{\mathbf{K}}
\providecommand{\mL}{\mathbf{L}}
\providecommand{\mM}{\mathbf{M}}
\providecommand{\mN}{\mathbf{N}}
\providecommand{\mO}{\mathbf{O}}
\providecommand{\mP}{\mathbf{P}}
\providecommand{\mQ}{\mathbf{Q}}
\providecommand{\mR}{\mathbf{R}}
\providecommand{\mS}{\mathbf{S}}
\providecommand{\mT}{\mathbf{T}}
\providecommand{\mU}{\mathbf{U}}
\providecommand{\mV}{\mathbf{V}}
\providecommand{\mW}{\mathbf{W}}
\providecommand{\mX}{\mathbf{X}}
\providecommand{\mY}{\mathbf{Y}}
\providecommand{\mZ}{\mathbf{Z}}

\providecommand{\va}{\mathbf{a}}
\providecommand{\vb}{\mathbf{b}}
\providecommand{\vc}{\mathbf{c}}
\providecommand{\vd}{\mathbf{d}}
\providecommand{\ve}{\mathbf{e}}
\providecommand{\vf}{\mathbf{f}}
\providecommand{\vg}{\mathbf{g}}
\providecommand{\vh}{\mathbf{h}}
\providecommand{\vi}{\mathbf{i}}
\providecommand{\vj}{\mathbf{j}}
\providecommand{\vk}{\mathbf{k}}
\providecommand{\vl}{\mathbf{l}}
\providecommand{\vm}{\mathbf{m}}
\providecommand{\vn}{\mathbf{n}}
\providecommand{\vo}{\mathbf{o}}
\providecommand{\vp}{\mathbf{p}}
\providecommand{\vq}{\mathbf{q}}
\providecommand{\vr}{\mathbf{r}}
\providecommand{\vs}{\mathbf{s}}
\providecommand{\vt}{\mathbf{t}}
\providecommand{\vu}{\mathbf{u}}
\providecommand{\vv}{\mathbf{v}}
\providecommand{\vw}{\mathbf{w}}
\providecommand{\vx}{\mathbf{x}}
\providecommand{\vy}{\mathbf{y}}
\providecommand{\vz}{\mathbf{z}}



% Greek Matrix bold
\providecommand{\mDelta}{\mat{\Delta}}
\providecommand{\mGamma}{\mat{\Gamma}}
\providecommand{\mLambda}{\mat{\Lambda}}
\providecommand{\mOmega}{\mat{\Omega}}
\providecommand{\mPhi}{\mat{\Phi}}
\providecommand{\mPi}{\mat{\Pi}}
\providecommand{\mPsi}{\mat{\Psi}}
\providecommand{\mSigma}{\mat{\Sigma}}
\providecommand{\mTheta}{\mat{\Theta}}
\providecommand{\mXi}{\mat{\Xi}}
\providecommand{\mSigmaNLM}{\mat{\Sigma}_{\mathrm{NLM}}}
\providecommand{\mSigmahat}{\mat{\widehat{\Sigma}}}

% Greeks Vector bold
\providecommand{\w}{\omega}
\providecommand{\valpha}{\vec{\alpha}}
\providecommand{\vbeta}{\vec{\beta}}
\providecommand{\vgamma}{\vec{\gamma}}
\providecommand{\vdelta}{\vec{\delta}}
\providecommand{\vepsilon}{\vec{\epsilon}}
\providecommand{\vvarepsilon}{\vec{\varepsilon}}
\providecommand{\vzeta}{\vec{\zeta}}
\providecommand{\veta}{\vec{\eta}}
\providecommand{\vtheta}{\vec{\theta}}
\providecommand{\vkappa}{\vec{\kappa}}
\providecommand{\vlambda}{\vec{\lambda}}
\providecommand{\vmu}{\vec{\mu}}
\providecommand{\vnu}{\vec{\nu}}
\providecommand{\vxi}{\vec{\xi}}
\providecommand{\vpi}{\vec{\pi}}
\providecommand{\vrho}{\vec{\rho}}
\providecommand{\vsigma}{\vec{\sigma}}
\providecommand{\vtau}{\vec{\tau}}
\providecommand{\vphi}{\vec{\phi}}
\providecommand{\vvarphi}{\vec{\varphi}}
\providecommand{\vchi}{\vec{\chi}}
\providecommand{\vpsi}{\vec{\psi}}
\providecommand{\vomega}{\vec{\omega}}









% Tilde
\providecommand{\wtilde}{\widetilde{w}}




% Tilde Matrix / Vector
\providecommand{\mAtilde}{\mat{\widetilde{A}}}
\providecommand{\mDtilde}{\mat{\widetilde{D}}}
\providecommand{\mWtilde}{\mat{\widetilde{W}}}
\providecommand{\vftilde}{\boldsymbol{\widetilde{f}}}
\providecommand{\vvtilde}{\boldsymbol{\widetilde{v}}}
\providecommand{\vxtilde}{\boldsymbol{\widetilde{x}}}
\providecommand{\vztilde}{\boldsymbol{\widetilde{z}}}

% Hat
\providecommand{\fhat}{\widehat{f}}
\providecommand{\zhat}{\widehat{z}}
\providecommand{\chat}{\widehat{c}}
\providecommand{\sigmahat}{\widehat{\sigma}}
\providecommand{\thetahat}{\widehat{\theta}}
\providecommand{\lambdahat}{\widehat{\lambda}}

% Hat Matrix / Vector
\providecommand{\vfhat}{\boldsymbol{\widehat{f}}}
\providecommand{\vzhat}{\boldsymbol{\widehat{z}}}
\providecommand{\vchat}{\boldsymbol{\widehat{c}}}
\providecommand{\vhat}{\widehat{v}}
\providecommand{\mAhat}{\mat{\widehat{A}}}
\providecommand{\vxhat}{\boldsymbol{\widehat{x}}}
\providecommand{\vuhat}{\boldsymbol{\widehat{u}}}
\providecommand{\vvhat}{\boldsymbol{\widehat{v}}}
\providecommand{\vubar}{\boldsymbol{\bar{u}}}
\providecommand{\vthetahat}{\boldsymbol{\widehat{\theta}}}
\providecommand{\vlambdahat}{\boldsymbol{\widehat{\lambda}}}


% Star
\providecommand{\fstar}{f^*}






% Standard 0 and 1
\providecommand{\vzero}{\vec{0}}
\providecommand{\vone}{\vec{1}}


% Operators
\providecommand{\conv}{\ast}
\providecommand{\circonv}[1]{\circledast_{#1}}
\providecommand{\Var}{\mathrm{Var}}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor}
\newcommand{\ceil}[1]{\left \lceil #1 \right \rceil}
\newcommand{\round}[1]{\left \lceil #1 \right \rfloor}

% Texts
\newcommand{\defequal}{\mathop{\overset{\mbox{\tiny{def}}}{=}}}
\newcommand{\subjectto}{\mathop{\mathrm{subject\, to}}}
\newcommand{\argmin}[1]{\mathop{\underset{#1}{\mbox{argmin}}}}
\newcommand{\argmax}[1]{\mathop{\underset{#1}{\mbox{argmax}}}}
\newcommand{\minimize}[1]{\mathop{\underset{#1}{\mathrm{minimize}}}}
\newcommand{\maximize}[1]{\mathop{\underset{#1}{\mathrm{maximize}}}}
\newcommand{\diag}[1]{\mathop{\mathrm{diag}\left\{#1\right\}}}
\newcommand{\MSE}{\mathrm{MSE}}
\newcommand{\trace}[1]{\mathop{\mathrm{Tr}\left\{#1\right\}}}
\newcommand{\erf}{\mbox{erf}}

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\newcommand{\by}[1]{\textcolor{blue}{[by]: #1}}

% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/Communication_Exp.tex <==
\begin{figure*}[!tb]
    \centering
    \vspace{1em}
    \includegraphics[width=0.65\textwidth]{Images/SVHN_Acc.pdf}
    \caption{The top-1 accuracy comparison under the same or similar computation and communication costs on the SVHN dataset. The ``Standard'' dash line means the same model activates all parameters during fine-tuning. The results on the SVHN dataset show a similar trend to previous experiments on Cifar-10 and Cifar-100 datasets. }
    \label{fig:SVHN results}
\end{figure*}
Figure~\ref{fig:SVHN results} shows the comparison results on the SVHN dataset. SVHN dataset is a digit classification dataset that contains over 600,000 RGB images. Under similar computational or communication costs, D2FT outperforms all baseline methods in fine-tuning performance but is minimally worse than the standard fine-tuning process, which shows the same trends as the experiments on Cifar-10 and Cifar-100 datasets in section~\ref{sec:results}. Interestingly, on this dataset, when computation or communication costs are below $60\%$, both magnitude dynamic pruning ("DPruning M" in the figure) and random scheduling ("Random" in the figure) methods fail to fine-tune the model effectively. Their fine-tuned model performance is even worse than that of the MoE methods.


==> sec/DesignDetails.tex <==
\textbf{Model Deployment:} We design to group the total $N$ devices to deploy the transformer base model. Since there are $B$ blocks in total, and each block contains $H$ attention heads. We distribute and deploy the entire model in two directions: layer-wise direction and width-wise direction. The block-wise direction is similar to the pipeline distributed, separating the entire model by its blocks. The width-wise separates the attention heads and activations for each block, and we suppose for each block $b$, there are $T$ (indexed by $t$) separation parts, where $T \leq H$. 
We use total $B\times T$ devices to contain the blocks of the transformer model. The width separation $t$ on each device for block $b$ can be seen as a sub-model with weight $W_{bt}$ (denoted as sub-model $W_{bt}$). We also need additional $2$ devices to deploy the patch embedding parts and the downstream dataset at the beginning and the linear projection parts at the end of the model. Therefore, we assign $N = B \times T$, with $2$ additional devices to deploy the entire model.

\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.88\linewidth]{Images/Layer-wise seperation.jpg}
    \caption{In the layer-wise separation illustration, we deploy the entire model separately by splitting its blocks. \by{this figure is trivial.. what novelty do we provide for the layer-wise partition? Emphasize on scheduling part. provide three options in the figure.}}
%\vspace{0.5em}
\end{figure}
\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.88\linewidth]{Images/One block design.jpg}
    \caption{The width-wise separation illustration. The dashed box with blue color means one transformer block. \by{this is also trivial... it can also be discussed in the experiments, the figure still needs to be more concise.} }
\label{fig: One_block}
\vspace{-0.5em}
\end{figure}

Similar to Shoeybi's work~\cite{shoeybi2019megatron}, we apply two all-reduce operations (one forward, one backward) for devices in each block. We do not apply the dropout layer and freeze norm layers to reduce the additional communication caused by splitting the dropout and norm layer during the training~\cite{korthikanti2023reducing}. \by{why?}
Figure~\ref{fig: One_block} illustrates our model deployment on devices. 

%Since the downstream task data are deployed on each device separately, we switch the device to provide data once it finishes providing its data. Since the two switched devices need to exchange their sub-model, we suppose we have sufficient non-computing memory storage (CPU memory cache) to store a sub-model and help it exchange.    

\textbf{Micro-Batch Computing Options:}
For every micro-batch $bch_{m}$ in a mini-batch $bch$, sub-model $W_{bt}$ have three options to operate it: 
\begin{itemize}
    \item \textbf{Forward-Backward (FB)}, \by{put detailed discussion here.}
    \item \textbf{Forward-Only (FO)},
    \item \textbf{Scaled-Shortcut (SS)}.
\end{itemize}
The forward-backward option means $bch_{m}$ do forward propagation on $W_{bt}$, and update it. The forward option means $bch_{m}$ only do forward propagation on $W_{bt}$ without update. Shortcut means $bch_{m}$ will not send to $W_{bt}$, bypass it to the next device. 

\textbf{Scaling the Shortcut Results \by{why do you put results here? also be consistent with the term.. shortcut or skipping? 
also, Skipping is not precise... 
How about ``Scaled Shortcut (SS)''?
}:}
\input{Scaling}

\textbf{Scoring Scheme:}
We aim to make a sub-model $W_b^h$ choose the most important inputs in every batch. To achieve our goal, we designed two scores, the forward score and the forward-backward score, to measure the importance of samples for each sub-model. Inspired by the works of pruning~\cite{kohama2023single}, we apply gradient and magnitude values as prediction scores to decide the importance of every micro-batch.  Each device (sub-model) chooses and assigns micro-batch computation operations with a higher prediction score. We will present more details in section~\ref{sec:scheduling}. To get the forward-backward score, we need an additional epoch for fine-tuning to make every micro-batch do the forward-backward operation before fine-tuning to get the gradients, but the model will not update. 

\textbf{Schduling Algorithm:} To average the workload balanced, we formulate the balancing problem as a Multi-Knapsack problem and apply a polynomial algorithm to solve it. We present our scheduling algorithm in section~\ref{sec:scheduling}. 

==> sec/DesignOverview.tex <==
Our purpose, which is to assign different samples activating on different sub-models of a large network, is a scheduling problem. We need to decide not only on the processed samples of each sub-model and keep the number of samples to each sub-model the same (balancing workload) but also on their processed operations. If we set an upper bound for the number of samples processed by a sub-model, we can make the scheduling balanced. Therefore, we can formulate our problem as a multi-knapsack problem. We set the importance prediction for each sub-model as the value in the multi-knapsack problem, the computation costs as the weights, and the computation capacity for devices as the knapsack volume. 

We create sub-models in our problem by splitting the large-scale pre-trained network depth-wise and width-wise, and each sub-model contains a portion of a layer or block. This distributed deployment is easy to achieve and can solve the memory overhead for a single device.  
For each sub-model, we give different options to process samples, which helps us sparsely activate the models with multiple values and weights. 
%Since we have different options, we need to set different values and weights in our multi-knapsack problem. 
Suppose we have options $1$, $2$, and not selected, we shall set two values $v1$ and $v2$ and two weights $w_1$ and $w_2$ to formulate our problem. Because we expect the workload for each device to be balanced, we give each device the same knapsack capacity $C$ in our problem and suppose there are a total of $K$ knapsacks (devices) indexed by $k$. Therefore, we can formulate our multi-knapsack problem as follows:
\begin{equation}
\label{eq:basic statement}
    \max\sum_k^K(\alpha v_1 + \beta v_2),
\end{equation}
\[
s.t. \quad \alpha w_1 + \beta w_2 \leq C, 
\]
\[
\alpha + \beta \leq 1, \quad \alpha, \beta \in \{0,1\}.
\]
Where $\alpha$ and $\beta$ means the number of samples choose option1 and option2. We will discuss the details in the following. 

%Because the multi-knapsack is an NP-complete problem~\cite{kan1993class}, we decoupled the multi-knapsack problem into knapsack problems to apply a polynomial algorithm, such as dynamic programming, to find the solutions. Like the pruning methods gradient evaluation, we can evaluate every sub-model's gradient independently to decouple the multi-knapsack problem from knapsack problems, where each device's micro-batch selection is a knapsack problem. We will discuss the details in section~\ref{sec:scheduling}.

==> sec/Design_Principle.tex <==
\subsubsection{Deploy the network distributed}
For a large-scale neural network, even one layer or block is large enough for most devices. Therefore, we split the model depth-wise (layers or blocks) and width-wise. For example, in a block of transformer model, the multiple attention heads can be deployed separately and split the feed-forward network (MLP layers) like tensor parallelism. With this framework, we can ensure the subnet memory cost is under a device's memory constraints. 

We split the input batch $B$ into several equal-size micro-batch $b$ to schedule each micro-batch using our algorithm.

\subsubsection{Option and Scoring settings} 
\input{Score_Scheme}

==> sec/Intro.tex <==
\section{Introduction}
\label{sec:intro}

Recently, fine-tuning foundation models have emerged as a novel learning paradigm within the field of machine learning and demonstrated remarkable performance gains across a wide range of machine learning tasks. Foundation models are extensively trained on vast datasets that cover a wide array of topics and knowledge domains, thereby facilitating a deep understanding of real-world concepts~\cite{devlin2018bert, liu2019roberta, raffel2020exploring, yang2019xlnet, sanh2019distilbert}. Leveraging this foundational understanding, these foundation models can be efficiently adapted to practical machine-learning tasks by fine-tuning their parameters from the pre-trained foundation models.
However, the enormous sizes of foundation models (e.g., GPT-4~\cite{bubeck2023sparks} with 1.8 trillion parameters, Vision Transformer~\cite{yuan2021tokens} with 86 million parameters) present a daunting challenge when adapting foundation models for fine-tuning on downstream tasks. 



% Since these models are already capable in a general sense, they can be fine-tuned with additional, smaller datasets to excel at specific tasks, i.e., downstream tasks. 

Fine-tuning a foundation model requires storing substantial amounts of data, including model parameters, intermediate activations, and gradient updates within the GPU memory. This poses a significant burden for most commercialized devices, such as laptops and desktops, equipped with consumer-grade GPUs due to their limited memory sizes.
Nevertheless, recent empirical findings have also shown that an increase in the number of parameters and layers typically enhances model performance~\cite{li2020train}. 
It is anticipated that the tension between the increasing size of neural networks and memory constraints will continue to be a prevalent trend, potentially exacerbated in the fine-tuning of foundation models, thereby hindering the full utilization of these models' capabilities.
To address this challenge, pipeline parallelism~\cite{belilovsky2020decoupled, yuan2022distributed, yuan2022decentralized} and tensor parallelism~\cite{shoeybi2019megatron,xu2021gspmd,xu2023efficient,bian2021maximizing} has widely adopted as promising solutions.
%\by{update model sharding to pipeline parallelism, see https://huggingface.co/transformers/v4.10.1/parallelism.html}
%\by{add tensor parallelism.}
To leverage the power of the crowd, pipeline parallelism splits the neural network into small pieces in a layer-wise manner to allocate the subnet into distributed devices, while tensor parallelism splits each tensor (weight matrix) into multiple chunks, with each residing on distributed devices. Both approaches allow each device to process a distinct set of parameters, reducing the memory requirements and computational load on individual devices. 
% train a neural network over distributed devices. 
% The layers or blocks of neural networks are partitioned into subnet works, thereby . 
% In this paper, we focus on Transformers. 
Take the transformer model~\cite{vaswani2017attention,dosovitskiy2020image} as an example; it consists of $12$ blocks where each sharing the same structure and having the same input/output size. Each block has two main components: a multi-head attention network and a feed-forward network. Each attention head calculates the weight independently, concatenates the results, and then sends it to the feed-forward network. Therefore, we can split a large-scale transformer model in different ways, e.g., by blocks (i.e., pipeline parallelism) or attention heads (i.e., tensor parallelism).
%it is possible to use each attention head independently and separate the feed-forward network to distributed training the model. \by{this is not sequential then.}
%\by{introduce the architecture of transformers and how it can be split into different attention modules.}
%Since transformers are composed of stacked layers, sequential model sharding can be applied to models with certain sizes (), making it one of the promising approaches for training increasingly large neural networks. 


% In this paper, we observe that, when adapting to downstream tasks, not all attention modules in foundation models are necessary for performing forward and backward propagation operations.

% Despite the benefit of memory reduction, model sharding and tensor parallelism introduce additional overheads in execution time, computational, communication, and energy consumption. Many recent works have been developed to mitigate these overheads. For example, pipeline parallelism methods~\cite{huang2019gpipe,narayanan2019pipedream,narayanan2021memory} have been widely investigated to reduce the training execution time. These methods are typically designed to minimize the idle time (\ie, pipeline bubbles) on each device by filling up the training pipeline between batches. However, given the dependency between layers and heads, it is still challenging to significantly reduce the execution time.

% The existing works mainly focus on conventional neural networks where all subnet and their corresponding devices must be involved in the whole training process. However, in the era of foundation models, such constraints are no longed necessary.
% mainly focuses on training these models from scratch.
% and aims to reduce the execution time of training via various pipeline parallelism methods~\cite{huang2019gpipe,narayanan2019pipedream,narayanan2021memory} to fill up the training pipeline and minimize the idle time on each device.
% one key benefit of large-scale neural networks - the nature of a foundation model - has not been well utilized. 
While existing methods offer the advantage of memory saving, they are mainly investigated in the traditional training paradigm, where models are always from scratch. The potential of foundation models in facilitating the fine-tuning process is fully exploited by the existing methods. 
It has been observed that it is effective to adapt to downstream tasks without fine-tuning all the parameters in foundation model~\cite{touvron2022three}. 
% As one key benefit of large-scale neural networks, to fine-tune a general-purpose foundation model on a downstream task, it is not necessary to update all the parameters~\cite{touvron2022three}. 
This intuition has inspired our initial design towards reducing the workload in the existing pipeline parallelism.
% We hypothesize that given a downstream training sample, no
We hypothesize that not all the attention modules in both forward pass and backward pass have significant contributions to fine-tuning a given training sample. Therefore, for each training sample, we can skip the operations on the specific subnet and their corresponding devices during fine-tuning, which largely saves computational and communication costs while preserving the fine-tuning accuracy.
First, to adapt to a specific downstream task, not all the parameters are required to be updated. Hence, the backward operations could be skipped on a specific subnet. 
% First, in the backward pass, it has been shown that not all the parameters and their gradients are required to be calculated and updated. Hence, we can skip the backward operations on specific subnet.
% First, given a downstream training sample, in the backpropagation, gradients of a part of subnet do not need to be computed. 
% , which largely saves the computational, communication, and energy costs.
Second, in the forward pass, our empirical results show that given a training sample, a specific subnet can be approximated by a linear function without affecting its performance. 
Then, the forward operations on these subnets (and their devices) can also be skipped, with minimal cost of running the linear function on the other devices.
Therefore, given a training sample, three options are sorted out for the subnet: i) performing the forward and backward operations, ii) performing the forward pass only, and iii) not performing any operations. We will detail the operations in Section~\ref{sec:operation selection}.

However, merely skipping operations may lead to significant imbalance issues among devices since a few subnets are more important than others, and more intensive workloads will be allocated to their corresponding devices. 
The devices with important subnets will then suffer from more intensive loads and become bottlenecks, significantly slowing down the entire system.

%\by{move these paragraphs of sparse training and MOE to related work.}
% Similar ideas have been developed in centralized training to reduce computational costs. For example, sparse training~\cite{han2015learning, lee2018snip, kohama2023single} removes some parameters in training. Mixture of Experts (MoE)~\cite{lepikhin2020gshard, zuo2021taming} allows only a few experts (subnet) to be involved in the training. However, these approaches only consider options i) and iii); the option of forward-pass only is not considered in their design. The pruning methods focus on compressing a large-scale network, using gradients to measure the importance of nodes. Hence, the training process needs all remaining nodes to do backpropagation, which considers a forward pass only unnecessary.  
% The subnets in MoE methods are used to fit different tasks. There is no need to provide knowledge of other tasks for a specific task. Therefore, the MoE methods also do not consider the option of forward pass only. Thus, none of them consider evaluating parameters to do only forward options.
%Including a forward-pass option will lead to a significant reduction in computation in distributed learning. 
%\by{this does not answer my question. Why forward-only is not considered in centralized training?}


%\by{we need to measure the imbalance workloads. check other works.}
% More importantly, as these methods are designed for a single machine, one of the key metrics in distributed learning - load-balancing - is not considered here. The accuracy-driven selection may lead to imbalanced workloads among participated devices, thus slowing down the overall training speed.

To address this challenge, we propose a framework called Distributed Dynamic Fine-Tuning (D2FT) that dynamically allocates learning operations across distributed devices for fine-tuning a foundation model on downstream tasks. 
Specifically, we first partition a neural network into multiple attention-based subnets and assign them to individual devices, ensuring each subnet fits within the device's memory capacity.
Accordingly, we formulate the scheduling as a multi-knapsack problem. The objective is to optimize the learning performance without overloading the workload on any devices by dynamically selecting appropriate learning options.
Our major contributions are four-fold:

\begin{itemize}[leftmargin=*]
\item We develop a new distributed learning framework (D2FT) that is memory and computation-friendly for recourse constraint devices.
%\vspace{-0.7em}
\item We propose three selection options to select important samples (micro-batch) to process for each subnet, reducing computation and communication costs over devices.
%\vspace{-2em}
\item We formulate a multi-knapsack problem for the load-balancing challenge and derive the solution.  
%\vspace{-0.7em}
\item The experiment results show that D2FT outperforms baseline methods, reducing the training computation cost by $40\%$ and training communication cost by $50\%$ with $1.2\%$ and $4.9\%$ accuracy drop on Cifar-10 and Cifar-100 datasets, respectively.
%\vspace{-0.5em}
%communication costs of tensors transformation with merely $0.9\%$ and $5.2\%$ top-1 accuracy drop on the Cifar-10 and Cifar-100 datasets.  \by{double check these numbers, write in this way: reduce the xx cost by xx\% ... see abstract}
\end{itemize}


==> sec/Scenario.tex <==
Suppose there are $N$ high-speed computing devices (such as GPUs) participating in the fine-tuning task, where the one input batch in the task is denoted as $B$. Each device has a similar but limited memory capacity. The trained model is a transformer base model, with $L$ (indexed by $l$) blocks in total, and the attention heads can be split into $H$ (indexed by $h$) vertical parts. We suppose all devices have the same processing speed and do not consider the latency between devices.

==> sec/Scheduling_Algorithm.tex <==
\input{Algorithm_new}
\input{Algorithm_2new}
In this part, we first transfer equation~\ref{eq:basic statement} to our scheduling problem statement, then reduce the complex multi-knapsack problem to an easier multi-knapsack problem and apply a dynamic programming algorithm in polynomial time to solve it. 

\textbf{Problem Formula:} We suppose for each forward propagation, the computation cost is $c$, and the backward propagation cost is $d$. For each micro-batch $b$, we add a mutually exclusive constraint that one sub-model could only choose one possible option. Our scheduling goal is to balance the workload for each sub-model, which means the total computation cost of processing micro-batches with each device (sub-model) computation capacity is denoted as $C_{(l,h)}$, and maximize the scores for all sub-models choices. Therefore, our multi-knapsack problem can be formulated as follows:
\begin{equation}
\label{eq:multi-knapsack}
    \max\sum_l^L\sum_h^{H}\sum_{b}^{B}({(l,h)}^{b}{Bs}_{k}^{b} + \beta_{(l,h)} {Fs}_{(l,h)}),
\end{equation}
\[
s.t. \sum_{b}^{B}(\alpha_{l,h}^{b}(c + d) + \beta_{l,h}^{b} c) \leq C_{l,h}, 
\]
\[
\alpha_{l,h}^{b} + \beta_{l,h}^{b} \leq 1, \quad \alpha_{l,h}^{b}, \beta_{l,h}^{b}\in \{0,1\}.
\]
The binary factor $\alpha_{l,h}^{b}$ and $\beta_{l,h}^{b}$ means the decision of choosing $FB$ option, $FO$ option or $NO$ option for a micro-batch $b$.

%\textbf{Problem Decoupling} 

%\textbf{Value Selection}
%1) why decouple this multi-knapsack
%2) if it is decoupled, is it equivalent to the original problem?
%we get some intuition from previous work.
%but we find that value selection is appropriate, we will minimize the impact and get approximate results
%3) new problem formulation.

%\textbf{two-stage knapsack}

\textbf{Problem Decoupling:} Since the multi-knapsack problem is an NP-Hard problem~\cite{kan1993class}, it is hard to find a polynomial time algorithm to find solutions. If we can decouple the multi-knapsack problem and simplify it to knapsack problems, we can solve it in polynomial time. Our idea is to evaluate the knapsack of each sub-model independently, which divides the multi-knapsack problem into $N$ knapsack problems, where $N$ is the participating device number. But a problem is whether the decoupling problem is equivalent to our problem in equation~\ref{eq:multi-knapsack}. 
%If the selection of each sub-model (knapsacks) is independent, our multi-knapsack problem is equivalent to knapsack problems. 
We get some intuition from previous works, such as one-shot pruning~\cite{lee2018snip,kohama2023single}. These works independently evaluate each parameter's gradient or magnitude value, which gives us solutions that we can evaluate gradient and magnitude values in our problem.
Therefore, we can simplify the multi-knapsack problem to multiple knapsack problems, in which every sub-model's selection is a knapsack problem. 
Hence, we maximize the score of every knapsack under its capacity, and the optimization problem for equation~\ref{eq:multi-knapsack} can be changed to:
\begin{equation}
\label{eq:multiple knapsacks}
    \max\sum_{b}^{B}\alpha_{l,h}^{b}{Bs}_{l,h}^{b} + \beta_{l,h}^{b} {Fs}_{l,h},\quad l\in L, h\in H
\end{equation}
\[
s.t. \sum_{b}^{B}(\alpha_{l,h}^{b}(c + d) + \beta_{l,h}^{b} c) \leq C_{l,h}, 
\]
\[
\alpha_{l,h}^{b} + \beta_{l,h}^{b} \leq 1, \quad \alpha_{l,h}^{b}, \beta_{l,h}^{b}\in \{0,1\}.
\]
We apply dynamic programming to solve equation~\ref{eq:multiple knapsacks}, where the dynamic programming builds a table where each cell represents the maximum value that can be achieved with a certain weight capacity and a certain number of items considered to find the best solution.

\textbf{Two-stage Scheduling:}
In our scheduling problem, we try to limit the number of micro-batches processed by each sub-model equally, where we try to give each sub-model an equal update during fine-tuning. But if we schedule the route by using all forward scores and backward scores, it is necessary to apply a scaler scaling the forward scores and backward scores. However, it is hard to find an appropriate scaler, and an inappropriate scaler can degrade the framework's performance. We prove this in section~\ref{sec:Two Stage}
%As an example, one sub-model may choose $2$ micro-batches to do $FB$ and $1$ micro-batch to do $FO$; the other may not choose micro-batches to do $FB$ but choose $7$ micro-batches to do $FO$. Although the total computation costs for these two devices are similar (suppose the backward computation cost is twice the forward computation cost), the first sub-models have been updated twice, but the second one updates nothing. 

Hence, we split the knapsacks (computation capacity) into two parts to calculate the forward and forward-backward computation costs separately. We set two computation capacities for each sub-model $W_{(l,h)}$: $CB_{(l,h)}$ for forward-backward computation and $CF_{(l,h)}$ for forward computation, where the capacity for the device deployed sub-model $W_{bt}$ follows
\[C_{l,h} = CF_{l,h} + CB_{l,h}.\]
Therefore, we can modify the equation~\ref{eq:multiple knapsacks} as:
\begin{equation}
\label{eq:multiple knapsacks new}
    \max\sum_{b}^{B}(\alpha_{l,h}^{b}{Bs}_{l,h}^{b} + \beta_{l,h}^{b} {Fs}_{l,h}),\quad l\in L, h\in H
\end{equation}
\[
s.t. \sum_{b}^{B}\alpha_{l,h}^{b}(c + d) \leq CB_{l,h},
\]
\[
\sum_{b}^{B}\beta_{l,h}^{b} c \leq CF_{l,h}, 
\]
\[
\alpha_{l,h}^{b} + \beta_{l,h}^{b} \leq 1, \quad \alpha_{l,h}^{b}, \beta_{l,h}^{b}\in \{0,1\}.
\]
Our algorithms are shown in Algorithm~\ref{Alg: Overall} and~\ref{Alg: DP}.

==> sec/Score_Scheme.tex <==
We set three possible options for a sub-model processing its input samples: 
\begin{itemize}
    \item forward-backward ($FB$),
    \item only forward ($FO$),
    \item not performing any operation ($NO$).
\end{itemize}
We learn to design the $FB$ and $NO$ options from the sparse training technique (e.g., pruning methods). Unlike the pruning methods that try to find a sub-model to substitute the entire large-scale network, our goal is to train the entire model by sparsely activating different parts for different inputs. Therefore, we designed the only forward ($FO$) option to give the activating sub-models knowledge of deactivating (no updates) sub-models during forward propagation. The new design can increase the network's performance after training, and we will show this in our experiments. 

Since we apply three selection options for each device, we design two scores for our algorithm to do scheduling. These scores reflect each micro-batch $b$ importance for every sub-model $W_{l,h}$.\\
\textit{Forward Score:} The value of the forward score ($Fs$) is the sum of the pre-trained weights' magnitude in sub-model $W_{l,h}$:
\[
{Fs}_{l,h} = \sum\| w\|, w\in W_{l,h}.
\]
This score decides whether a micro-batch will be forward processed by sub-model $W_{l,h}$.\\
\textit{Backward Score:} The value of Backward score ($Bs$) is the sum of the weights' gradient in sub-model $W_{l,h}$ for different micro-batch $b$ of $Loss$:
\[
{Bs}_{l,h}^{b} = \sum \frac{\partial Loss}{\partial w}, w\in W_{l,h}.
\]
Our idea comes from the scoring scheme from pruning methods. Since a large weight magnitude is important to the final results, Han et al.~\cite{han2015learning} remain the necessary weights iteratively according to their magnitude. Since our scoring scheme is a one-time scoring, which scores for each micro-batch before training and will not update the score during fine-tuning, we decided to use the sum weights' magnitude as the forward score of each sub-model. 
Meanwhile, inspired by the work of Lee et al.~\cite{lee2018snip}, where they set the gradient value of each weight as the saliency importance score to prune the model, we can apply the gradient value caused by different micro-batches as the basis to decide each micro-batch forward-backward computing options. 

\subsubsection{Linear transformation for not performing}
Not performing any operation $NO$ decreases the model performance because it shortcuts a sub-model result and sends the residual value to the next sub-model. To mitigate the influence of $NO$, we add a linear transformation function on all sub-models input once the previous sub-model $W_{l,h}$ has been skipped (scheduled $NO$ option) to mitigate the model performance decreasing. This linear transformation function can be written as $Ax + B + 0$,
where x is the residual input, and A and B are two trainable parameters. The $0$ means the result of the $NO$ option. We initialize $A = 1$ and $B = 0$ while training. 

==> sec/macro.tex <==
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} \def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\newcommand{\figref}[1]{Figure~\ref{fig:#1}}% type "\figref{}" to reference figure
\newcommand{\tabref}[1]{Table~\ref{tab:#1}} % type "\tabref{}" to reference table
\newcommand{\itmref}[1]{[\ref{itm:#1}]}     % type "\itmref{}" to reference item
\newcommand{\eqnref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
 
% \newcommand{\MR}[1]{\multirow{2}{*}{#1}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\n}{\mbox{\qquad}}              % type "\n" to indent at the begin of the line
\newcommand{\red}[1]{{\color{red}#1}}

%% editing comment
\newcommand{\ignore}[1]{}   % ignore this

\newcommand{\TODO}[1]{\textcolor{red}{[TODO]\{#1\}}}
\newcommand{\by}[1]{\textcolor{blue}{[by]: #1}}
